Profiling Irony & Stereotype: Exploring Sentiment, Topic, and Lexical Features

Social media has become a very popular source of information. With this popularity comes an interest in systems that can classify the information produced. This study tries to create such a system detecting irony in Twitter users. Recent work emphasize the importance of lexical features, sentiment features and the contrast herein along with TF-IDF and topic models. Based on a thorough feature selection process, the resulting model contains specific sub-features from these areas. Our model reaches an F1-score of 0.84, which is above the baseline. We find that lexical features, especially TF-IDF, contribute the most to our models while sentiment and topic modeling features contribute less to overall performance. Lastly, we highlight multiple interesting and important paths for further exploration.

==> Sections/Questions.tex <==
\textbf{Question 2}: \textit{In previous years, the shared task focused on spreaders of fake news or hate speech. Considering your experience, do you think that the features that you used would be useful for the detection of other types of information spreaders (either fake news, hate speech, or both)? Would you expect any of your features only to be good for detecting irony and stereotype spreaders?}

As defined at the beginning of this paper, irony can be considered as the way of describing something literally while meaning the opposite. Fake news can be defined as dis- (false information that one deliberately spreads) and -misinformation (false information that one spreads without knowing that it is not true) on the internet or social media \cite{zhang_overview_2020, gelfert_fake_2018}. Hate speech is characterized by communication that incites, threatens, or discriminates against a person or group because of for example their race, gender, or sexual orientation \cite{tontodimamma_thirty_2021}. Common for all three is that i) they can promote discriminating behaviour including for example racism, panic, homophobia and xenophobia \cite{alam_survey_2021, tontodimamma_thirty_2021}, ii) they are commonly spread and used on social media for example, on Twitter \cite{poletto_resources_2021, geeng_fake_2020}, and iii) irony, fake news or hate speech, can all be a case of user profiling, i.e we can consider a user as one producing irony, fake news or hate speech or one that does not.

Because they can all be internet-based in the form of posts, they become more comparable in terms of which approaches work in the detection of them. Within our solution to this year’s shared task, some of the used features have been beneficial in other user profiling task. Among these are POS-unigrams, mean tweet length and TF-IDF \cite{rangel_overview_2019}. These features provide a detailed insight to the way language is used (e.g. fake news spreader have an increased use of second person \cite{rashkin_truth_2017}).

Our other features are related to the specific aspects expected of irony through topic modelling and sentiment analysis. The applicability of topic modelling depends on the phenomenon. \\
In relation to fake news, very specific topics are dealt with, e.g. viruses or presidential campaigns \cite{rashkin_truth_2017}, making a topic model useful. However, if they are compared to regular news, there will be a lot of overlap. \\
\indent With regards to hate speech, it lies in the definition that it is directed towards specific communities, which we could perhaps capture with a topic model. Considering our own results, it is however also possible that the TF-IDF can function in such way. 

We also extracted sentiment contrast, variance, and disagreement. These are used specifically for the irony domain and its characteristics as already suggested in early years \shortcite{kreuz_two_1995, utsumi_verbal_2000}. Therefore, we expect they will not be advantageous for detecting fake news or hate speech. However, sentiment itself can be relevant. In fake news, one could imagine that texts express extreme values of sentiment, both positive and negative, like a cure against a virus \cite{zhang_overview_2020}. In this way, sentiment can assist in detecting such texts. Hate speech texts, on the other hand, will most likely occur in the negative extreme. Including emotion analysis in a model could benefit the detection as in \citeA{pineda_profiling_2021}. 

A topic model might in interaction with for example sentiment be strengthened. This scenario could be especially relevant for hate speech. If a text taps into a topic within sexual orientation, it can be both hate speech and non-hate speech. However, if the text taps into that topic and is highly negative, it is more certain that it is a case of hate speech. 

To conclude, we think that some of the features we used for irony detection can also be applied for profiling spreaders of fake news or hate speech such as TF-IDF, POS-unigrams, mean tweet length and sentiment scores. However, features specifically designed for capturing irony (based on the definition of irony) we deem less relevant for profiling fake news or hate speech spreaders. 

\newpage
\textbf{Question 3}: \textit{Give an account of what emotion and affect lexicons are, provide examples of the way they are built, and explain the way they are used in NLP. In particular, discuss how they may be applied to the task of irony detection and the profiling of irony spreaders.}

Emotion can be defined as "a conscious mental reaction" \shortcite{merriam-webstercom_emotion_2022} and affect as "the conscious emotion that occurs in reaction to a thought or experience" \shortcite{merriam-webstercom_affect_2022} even though the literature doesn't agree on a uniform definition \shortcite{mulligan_toward_2012}.

The lexicons accompanying both are a collection of words that reflect those "mental reactions" or "the conscious emotion" and are widely used as a resource for emotion and affect analyses \shortcite{yang_building_2007, hwan_automatic_2006}. These can be either categorical-based \shortcite{shaver_emotion_1987, abdaoui_feel_2017} or dimension-based \shortcite{mohammad_obtaining_2018}. Earlier, many lexicons focused on differentiating positive and negative words, but later approaches attempt to construct more fine-grained lexicons differentiating between five to eight emotions \shortcite{do_korean_2015, jurafsky_speech_2009}. 

Affect lexicons can be constructed by crowd-sourcing, semi-supervised induction or supervised learning \cite{paggio_language_2022}. An example of an affect lexicon that is constructed by means of crowd-sourcing is the dimension-based NRC Valence Arousal Dominance (VAD) lexicon \cite{mohammad_obtaining_2018}. Here, words are provided with scores for valence, arousal and dominance, making it a dimension-based approach \cite{russell_circumplex_1980}. The NRC VAD lexicon is built by applying the best-worst scaling method \cite{louviere_best-worst_2015}. This method presents a set of words and the participant is to determine which word is most and least related to an emotion \cite{jurafsky_speech_2009}.

NLP is concerned with how systems can process human language as well as the human-computer interaction \cite{jurafsky_speech_2009}. Over the last years the field has become large and popular and therefore the applications of affect lexicons vary broadly. However, affect lexicons are mostly used in NLP for sentiment analysis, which aims to capture the sentiment of written text. For example, the sentiment analyzer VADER is based on an affect lexicon that is called VADER’s sentiment lexicon \cite{hutto_vader_2014} and can be used to capture the positive, neutral and negative sentiment of a word. Then, by passing each word from text documents such as tweets through the lexicon, one can obtain the affect a word contains and have an idea of the distribution of affect and sentiment within the collection of texts.

As demonstrated in our solution to the shared task, sentiment can be a predictor of irony if one considers sentiment as relevant \cite{joshi_automatic_2016}. 
Furthermore, affect lexicons can be explored to construct more complex sentiment features that might predict sentiment. E.g., we define sentiment disagreement as the squared difference between two sentiment analyzers for the same tweet (see method Section \ref{sec:methods}). Another way to construct sentiment disagreement is to predict sentiment scores of a tweet based on two different affect lexicons.

In conclusion, emotion and affect lexicons are dictionaries where emotion and affect values for specific words can be looked up. They can be built in several ways, where for some approaches it is very expensive to collect affect scores (crowd-sourcing), as for other approaches it requires large corpora of text that inherently have an emotion related to it, like reviews (supervised learning). Affect lexicons can applied in NLP in sentiment analysis. This is related to irony detection as sentiment scores can be a predictor of irony. 
